A Concurrency Problem with Exponential DPLL(T) Proofs

Many satisfiability modulo theories solvers implement a variant of the DPLL(T ) framework which separates theory-specific reasoning from reasoning on the propositional abstraction of the formula. Such solvers conclude that a formula is unsatisfiable once they have learned enough theory conflicts to derive a propositional contradiction. However some problems, such as the diamonds problem, require learning exponentially many conflicts. We give a general criterion for establishing lower bounds on the number of theory conflicts in any DPLL(T ) proof for a given problem. We apply our criterion to two different state-of-the-art symbolic partial-order encodings of a simple, yet representative concurrency problem. Even though one of the encodings is asymptotically smaller than the other, we establish the same exponential lower bound proof complexity for both. Our experiments confirm this theoretical lower bound across multiple solvers and theory combinations.

==> related.tex <==
\section{Related Work}
\label{section:related-work}

Over the last ten years, much research has gone into symbolic partial-order encodings for concurrency, e.g.~\cite{YGLS2004,GYS2004,BAM2007,WKGG2009,TVD2010,BWBOS2011,AKT2013,HK2015}. Some of these works (e.g.~\cite{BWBOS2011}) use nonstandard constraint solvers for first-order relational logic. Previous experimental studies~\cite{AKT2013} focused on a particular SAT solver, whereas our experiments consider a range of SMT solvers and combinations of SMT theories. We setup the experiments independent of a particular language or hardware semantics, e.g.~\cite{SSONM2010,SVZJS2011,BOSSW2011,AMSS2012}. A comprehensive treatise on the theory of SAT/SMT-based partial-order encodings~\cite{HK2015} discusses related work in the so-called `true concurrency' literature.

